Uniform Interpolants in EUF: Algorithms using DAG-representations

The concept of uniform interpolant for a quantifier-free formula from a given formula with a list of symbols, while well-known in the logic literature, has been unknown to the formal methods and automated reasoning community for a long time. This concept is precisely defined. Two algorithms for computing quantifier-free uniform interpolants in the theory of equality over uninterpreted symbols (EUF) endowed with a list of symbols to be eliminated are proposed. The first algorithm is non-deterministic and generates a uniform interpolant expressed as a disjunction of conjunctions of literals, whereas the second algorithm gives a compact representation of a uniform interpolant as a conjunction of Horn clauses. Both algorithms exploit efficient dedicated DAG representations of terms. Correctness and completeness proofs are supplied, using arguments combining rewrite techniques with model theory.

==> app.tex <==
\section{Appendix}\label{app}

In this Appendix we report the missing proofs from the different sections.


\subsection{Proofs of Section \ref{sec:cond}}


\vskip 2mm\noindent
\textbf{Lemma \ref{lem:oneside}} \emph{For every set of clauses $S$ and for every 
$\uw$-conditional DAG $\delta$ built out of $S$, 
%we have that 
the formula
$$
\bigwedge S \to \phi_{\delta}
$$
is logically valid.
}
\vskip 1mm
\begin{proof}
%silvio 16/2 various indexes _i were missed
 We prove that $ \bigwedge S \to \phi_{\delta}^i$ is valid by induction on $i$. The base case is clear. For the case $i\leq s$, proceed, e.g., in natural deduction as follows: %ale: why 'natural deduction'? it seems like the name of the proof calculus
 %silvio because this argument strictly follows a natural deduction proof (following say sequnt calculus wouls be more difficult to explain); I added ``e.g. in natural deduction'' to say that the reader may use the calculus he prefers
 assume $S, \Gamma_i$ and $\tilde w_i=t_i$ in order to prove $\phi_{\delta}^{i+1}(\tilde w_i/w_i)$. Since $\Gamma_i\to w_i=t_i\in S$, then 
 by implication elimination you get $w_i=t_i$ and also $w_i=\tilde w_i$ by transitivity of equality. Now
 you get what you need from induction hypothesis and equality replacement.
\end{proof}

\subsection{Proofs of Section \ref{sec:completeness}}

We report now the full proof of correctness and completeness of the Tableaux Algorithm:

\vskip 2mm\noindent
\textbf{Theorem~\ref{thm:tab-cover}}
\emph{Suppose that we apply the  algorithm of Subsection~\ref{subsec:tabalg} to the
 primitive formula 
 $\exists \ue(\phi(\ue, \uz))$ 
 and that the algorithm terminates with its branches 
 %have the dag-primitive format~~\eqref{eq:primitive}; if 
 %the above algorithm, initiated with~\eqref{eq:primitive}, terminate  its branches  
 in the states 
$$
\delta_1(\uy_1,\uz)\wedge  \Phi_1(\uy_1,\uz) \wedge \Psi_1(\ue_1, \uy_1, \uz),
~~~\dots,~~~ 
\delta_k(\uy_k,\uz)\wedge  \Phi_k(\uy_k,\uz) \wedge  \Psi_k(\ue_k, \uy_k, \uz)
$$ 
then the UI of $\exists \ue(\phi(\ue, \uz))$ in \EUF is the \emph{unravelling} of the formula
\begin{equation}
 \bigvee_{i=1}^k \exists \uy_i ~(\delta_i(\uy_i, \uz) \wedge \Phi_i(\uy_i, \uz))~~.
\end{equation}
}

\begin{proof} Since $\exists \ue(\phi(\ue, \uz))$ is logically equivalent to $\bigvee_{i=1}^k \exists \uy_i ~(\delta_i(\uy_i, \uz) \wedge \Phi_i(\uy_i, \uz)\wedge \exists \ue_i \Psi_i(\ue_1, \uy_1, \uz))$, it is sufficient to check that if a formula like~\eqref{eq:primitive} is terminal (i.e. no rule applies to it) then its UI is $\exists \uy ~(\delta(\uy, \uz) \wedge \Phi(\uy, \uz))$.
%
To this aim, we apply Lemma~\ref{lem:cover}: we pick a model  $\cM$ satisfying $\delta(\uy, \uz) \wedge \Phi(\uy, \uz)$ via an assignment $\cI$ to the variables $\uy, \uz$\footnote{Actually the values of the  assignment $\cI$ to the $\uz$ uniquely determines the values of  $\cI$ to the $\uy$.} and we show that $\cM$ can be embedded into a model $\cM'$ such that, for a suitable extensions $\cI'$ of $\cI$ to the variables $\ue$, we have that $(\cM', \cI')$ satisfies also $\Psi(\ue, \uy, \uz)$.
%
What we need (by Robinson Diagram Lemma) is to find a model for the following set of literals 
\begin{equation}\label{eq:TR}
\Delta(\cM)\cup \Psi  \cup \{  a= \tilde a\}_{a\in \uy\cup \uz}
\end{equation}
where $\tilde a$ is the value of $a$ under the assignment $\cI$ (here all variables in~\eqref{eq:TR} are seen as constants, so~\eqref{eq:TR} is a set of ground literals).  
We can orient the equalities in~\eqref{eq:TR} by letting function symbols having bigger precedence 
over constants and by letting $a$ having bigger precedence over $\tilde a$. Normalizing~\eqref{eq:TR} replaces $a$ with $\tilde a$ in $\Psi$: call $\tilde \Psi$ the resulting set of literals. Now we claim that all oriented equalities in $\Delta(\cM)\cup \tilde\Psi  \cup \{  a= \tilde a\}_{a\in \uy\cup \uz}$ form a canonical rewriting system. This is due to Remark~\ref{rmk:terminal}: in fact (let $\tilde e_i$ be $e_i$ for all $e_i\in \ue$) if $f(a_1, \dots, a_n)$ and $f(b_1, \dots, b_n)$ both occur in $\Psi$, it cannot happen that $f(\tilde a_1, \dots, \tilde a_n)$ and $f(\tilde b_1, \dots, \tilde b_n)$
are the same term because the $\ue$ are already in normal form and because $\cM\models \Phi$ (and hence also 
$\cM\models \tilde \Phi$). In addition, if $f(a_1, \dots, a_n)$ occurs in $\Psi$, then one of the $a_i$ belongs to $\ue$, hence rules from $\tilde \Psi$ and $\Delta(\cM)$ cannot superpose.
%
Since all oriented equalities in $\Delta(\cM)\cup \tilde\Psi \cup \{  a= \tilde a\}_{a\in \uy\cup \uz}$ form a canonical rewriting system, the inequalities in $\Delta(\cM)\cup \tilde\Psi$ are in normal form and  we can apply Lemma~\ref{lem:canonic} to get the desired $\cM'$. 
\end{proof}

We now move on to the full proof of correctness and completeness of the Conditional Algorithm
In order to prove Theorem~\ref{thm:main}, we first need to prove the following Lemma:

\begin{lemma}\label{lem:pers}
If the clauses $\Gamma \to f(a_1, \dots, a_h)= b$ and $\Gamma'\to f(a'_1, \dots, a'_h)= b'$ both belong to $S_3$
 %silvio 16/2
 %I added next line; in fact without it, for the Lemma to be correct we should produce trivial clauses like a_1=a_1, \dots, a_h=a_h \to b=b from a single atom f(a_1, \dots, a_h)= b$ in the input - which of course we do not want to do!!! The actual formulation of the lemma is obviously sufficient for the completeness proof
 %
 and $b$ is not the same term as $b'$, 
 then $S_3$ contains also a clause subsuming the clause
 \begin{equation*}
 \Gamma, \Gamma', a_1=a'_1, \dots, a_h=a'_h \to b=b'
\end{equation*}
\end{lemma}

\begin{proof}
 By induction on the number $K$ of applications of the  rewriting rule of Step 2 needed to derive $\Gamma \to f(a_1, \dots, a_h)= b$ and $\Gamma'\to f(a'_1, \dots, a'_h)= b'$. If $K$ is 0, the claim is clear by the instruction of Step 1. Suppose that $K>0$ and let $\Gamma'\to f(a'_1, \dots, a'_h)= b'$ be obtained from $\Gamma_1\to e_i= e_j$ by rewriting $e_j$ to $e_i$ from some clause $C$. We need to distinguish cases depending on the position $p$ of the rewriting. All cases being treated in the same way, suppose for instance that $p$ is in the antecedent,\footnote{ 
 Here you are another subtle case, where $p$ is in the consequent.
 %silvio 16/2 added footnote to cover trivial new case
 If $b'$ is  the same term as $b$ and we rewrite it, then $b'$ is $e_j$ and $\Gamma_1\to e_i= e_j$ is the clause we are looking for.
 }  so that $C$ is $\Gamma_2\to f(a'_1, \dots, a'_h)= b'$ and that $\Gamma'\to f(a'_1, \dots, a'_h)= b'$ is $\Gamma_1,\Gamma_2[e_i]_p\to f(a'_1, \dots, a'_h)= b'$. Then by induction hypothesis $S_3$ contains a clause subsuming 
 $$
 \Gamma,  \Gamma_2, a_1=a'_1, \dots, a_h=a'_h \to b=b'
 $$
 and rewriting with $\Gamma_1\to e_i= e_j$ produces 
 $$
 \Gamma, \Gamma_1,  \Gamma_2[e_i]_p, a_1=a'_1, \dots, a_h=a'_h \to b=b'
 $$
 as required.
\end{proof}

\vskip 2mm\noindent
\textbf{Theorem~\ref{thm:main}}\emph{
 Let $S_3$  be obtained as in Steps 1-2 from  $\exists \ue\, \phi(\ue, \uz)$. Then the conjunction of all possible $ \phi_{\delta}$ (varying $\delta$ among the  conditional DAGs that can be built out of $S_3$) is a UI of $\exists \ue\, \phi(\ue, \uz)$ in \EUF. 
}

\begin{proof}
 We use Lemma~\ref{lem:cover}. Condition (i) of that Lemma is ensured by Lemma~\ref{lem:oneside} above because $\bigwedge S_3$ is logically equivalent to $\phi$. So let us take a model $\cM$ and elements $\tilde \ua$ from its support such that we have $\cM\models \bigwedge_{\delta} \phi_{\delta}$ under the assignment of the $\tilde \ua$ to the parameters $\uz$. We need to expand it to a superstructure $\cN$ in such a way that we have $\cN \models \bigwedge S_1$, under some assignment to $\uz, \ue$ extending the assignment $\uz\mapsto \tilde \ua$
 (recall that $\bigwedge S_1$ is logically equivalent to $\phi$ too).
 From now on, we consider the assignment $\uz\mapsto \tilde \ua$ fixed, so that when we write $\cM\models C$ for a clause 
 %silvio 16/2 $C(\uy)$ 
 $C(\uz)$ 
 we mean that $\cM\models C$ holds under the assignment $\uz\mapsto \tilde \ua$.
 
 Notice that every $\uw$-conditional DAG $\delta$ extracted from $S_3$ (let it be given by the clauses~\eqref{eq:cDAG})
 is naturally equipped with a substitution $\sigma_{\delta}$ which is given in DAG form by
$
w_1 \mapsto t_1, ~\dots,~  w_s \mapsto t_s.
$
 We say that $\delta$ is \emph{realized} in $\cM$ iff 
 we have that
 $$
 \cM \models \bigwedge \Gamma_1\sigma_{\delta}, \dots, \cM \models \bigwedge \Gamma_s\sigma_{\delta}
 $$
 Let $\delta$ be a $\uw$-conditional DAG which is realized in $\cM$  and let it be maximal %such
 with this property
  (a $\uw$-conditional DAG $\delta$ is said to be bigger than a $\uw'$-conditional DAG $\delta'$ iff $\uw$ includes  $\uw'$ - the inclusion is as sets, the order is disregarded). Since $\cM\models \phi_{\delta}$ and $\delta$ is realized in $\cM$, it is clear that all $L_{\uw}$-clauses from $S_3$ (hence also  all $L_{\uw}$-literals from $S_1$) are true in $\cM$. Let $\uu=u_1, \dots, u_k$ be the variables from $\ue\setminus \uw$ and let $S_{\uu}$ be the literals from $S_1$ which are not $L_{\uw}$-literals. 
 %
What we need (by Robinson Diagram Lemma) is to find a model for the following set of literals 
\begin{equation}\label{eq:R}
\Delta(\cM)\cup S_{\uu}\cup \{  w_i= \tilde b_i\mid i=1, \dots, s\} \cup \{  z_i= \tilde a_i\mid i=1, \dots, M\}
\end{equation}
where $\tilde b_i$ is the value of $w_i\sigma_{\delta}$  under the assignment $\uz\mapsto \tilde \ua$.
We orient the functional equalities in~\eqref{eq:R} from left to right and the equalities $w_i= \tilde b_i$
also from left to right.  The $\ue$ are ordered as $e_1> \cdots > e_N$ and are bigger than the constants naming the elements of $\vert\cM\vert$; function symbols are bigger than constant symbols. 
We show that the ground Knuth-Bendix completion of~\eqref{eq:R} 
 cannot produce any inconsistent literal of the kind $t\neq t$ (this completes the proof of the Theorem).
 
 First notice that the rules $\{  w_i= \tilde b_i\mid i=1, \dots, s\} \cup \{  z_i= \tilde a_i\mid i=1, \dots, M\}$ simply eliminates the $\uw$ and the $\uz$  from $S_{\uu}$ (they become inactive after such normalization steps). Let $\tilde S_{\uu}$ be the set of equalities resulting after this elimination. It turns out that $\tilde S_{\uu}$ can only contains equalities of the kinds
 \begin{equation}\label{eq:11}
 f(a_1, \dots, a_h)= a
\end{equation}
\begin{equation}\label{eq:21}
 u_j\neq a
\end{equation}
where $a_1, \dots a_h, a$ can be either among the $\uu$ or constants naming elements of $\vert \cM\vert$. 
However some of the $\uu$ must be among $a_1, \dots, a_h$ for each equality of the kind~\eqref{eq:11}  because atoms not containing the $\uu$ are removed by $\Delta(\cM)$ and atoms like $u_i=t$ (where $t$ does not contain any of the $\uu$) cannot be there because $\delta$ is maximal. 
During completion, 
 in addition to these kinds of atoms, only atoms of the kind 
 \begin{equation}\label{eq:31}
  u_i= u_j 
 \end{equation}
can possibly be produced. This is a consequence of the next Lemma.
Below we say that a tuple of atoms $\Gamma$ is \emph{realized in $\cM$} iff the $\Gamma$ are $L_{\uw}$-atoms and $\cM\models \bigwedge \Gamma\sigma_{\delta}$; similarly we say that a literal $\Theta$ is \emph{conditionally realized in $\cM$} if there exists  $\Gamma$ realized in $\cM$ with $\Gamma\to \Theta\in S_3$ (if $\Theta$ is a negative literal, $\Gamma\to \Theta$ stands for $\Gamma,\neg \Theta\to\ $).

\begin{lemma}
 Suppose that a literal $\Lambda$\ is produced during the completion of~$\tilde S_{\uu}$. Then 
 it must be of the kinds~\eqref{eq:11},~\eqref{eq:21},~\eqref{eq:31}. Moreover there exists a literal $\Lambda'$ such that (i) $\Lambda'$ is conditionally realized in $\cM$;  (ii) $\Lambda$ is obtained from $\Lambda'$ by rewriting $\uz, \uw$ respectively to $\tilde \ua, \tilde \ub$. 
 %, and by rewriting some of the $v_j\in \uu$ to some other $v_{j'}\in \uu$ in such a way that $j>j'$ and in such a way that  $v_j = v_{j'}$ is conditionally true in $\cM$. 
\end{lemma}

\begin{proof}%\todo{Maybe I shall expand a bit this proof}
By straightforward case analysis; we analyze the most interesting case given by the superposition of two rules of the kind~\eqref{eq:11}. Suppose that
\begin{equation*}
 f(a_1, \dots, a_h)= a~~{\rm and}~~f(a_1, \dots, a_h)= b
\end{equation*}
produce the equality  $a=b$. Then by induction hypothesis, there are in $S_3$ two clauses like
$$
\Gamma'\to f(a'_1, \dots, a'_h)= a', ~~~\Gamma''\to f(a''_1, \dots, a''_h)= a''
$$
with $\Gamma', \Gamma''$ realized in $\cM$, with $a'_1, \dots, a'_h,a'$ rewritable (using 
$\uz, \uw \mapsto \tilde \ua, \tilde \ub$) to $a_1, \dots, a_h,a$, respectively, and with $a''_1, \dots, a''_h,a''$ also rewritable (using 
$\uz, \uw \mapsto \tilde \ua, \tilde \ub$) to $a_1, \dots, a_h,b$, respectively. By Lemma~\ref{lem:pers}, $S_3$ contains a clause subsuming 
\begin{equation}\label{eq:t}
\Gamma', \Gamma'', a_1'=a''_1, \dots, a'_h= a''_h \to a'=a'' 
\end{equation}
which is as required because $\Gamma', \Gamma'', a_1'=a''_1, \dots, a'_h= a''_h$ is realized in $\cM$ and $a'=a''$ rewrites (using 
$\uz, \uw \mapsto \tilde \ua, \tilde \ub$) to $a=b$. It remains to check that $a=b$ is of the kind~\eqref{eq:31}. If both $a',a''$ taken from the consequent of~\eqref{eq:t} belong to $\uz\cup \uw$, then since the antecedent of~\eqref{eq:t} is realized in $\cM$
%silvio 16/2 added next line 
and~\eqref{eq:t} belongs to $S_3$,
 $a$ and $b$ must be the same element from $\vert \cM\vert$, so that $a=b$ is a trivial identity (which does not enter into the completion). It cannot be that only one between
$a'$ and $a''$ belongs to $\uz\cup \uw$ (the other one being from $\uu$) because $\delta$ is maximal among conditional DAGs realized by $\cM$
and thus it  cannot be properly enlarged by adding it the additional conditional definition which would be supplied by~\eqref{eq:t}. Thus it must be the case that both $a', a''$ are from $\uu$, which implies that they cannot be rewritten  (using 
$\uz, \uw \mapsto \tilde \ua, \tilde \ub$), so that $a'$ is $a$, $a''$ is $b$ and $a=b$ is of the 
kind~\eqref{eq:31}. 
\end{proof}
\emph{Proof of Theorem~\ref{thm:main} (continued)}. Once $\tilde S_{\uu}$ (standing alone) is completed, only literals of the kinds~\eqref{eq:11},~\eqref{eq:21},~\eqref{eq:31} are produced.
No completion inference is possible between literals  of the kinds~\eqref{eq:11},~\eqref{eq:21},~\eqref{eq:31}
on one side and literals 
%With such literals, no rule 
from  $\Delta(\cM)\cup  \{  w_i= \tilde b_i\mid i=1, \dots, s\} \cup \{  z_i= \tilde a_i\mid i=1, \dots, M\}$ on the other side; hence the completion of  $\tilde S_{\uu}$ alone, once joined to $\Delta(\cM)\cup  \{  w_i= \tilde b_i\mid i=1, \dots, s\} \cup \{  z_i= \tilde a_i\mid i=1, \dots, M\}$ yields a completion of~\eqref{eq:R}. The only possible inconsistencies that can arise are given by  literals of the kind $u_i\neq u_i$.
Suppose that indeed one such a literal $u_i\neq u_i$ is produced during the completion of $\tilde S_{\uu}$. Applying the above lemma,
there should be 
%literals $u_{j_1}\neq u_{j_2}$, $u_{j_1}=u_i$,
%$u_{j_2}=u_i$, all conditionally true in $\cM$. This would imply, by the rewriting rule of Step 3, that 
%$u_i\neq u_i$ would also be conditionally true in $\cM$. But
%this would mean that $S_3$ should contain 
in $S_3$
a clause like $\Gamma, u_i=u_i\to \ $  (i.e.  after simplification, a clause like $\Gamma \to \ $) with $\Gamma$ being realized in $\cM$. The last %AGapril: modified 'the latter', I wrote 'the last' instead
means that $\cM\models \bigwedge\Gamma\sigma_{\delta}$. This cannot be, because $\Gamma \to \ $ is a $L_{\uw}$-clause from $S_3$: in fact, we have that $\cM\models \phi_{\delta}$ and that $\delta$ is realized in $\cM$, which imply that $\cM\models C\sigma_{\delta}$ holds for every $L_{\uw}$-clause from $S_3$ by the definition of $\phi_{\delta}$. In particular, we should have  $\cM\models \neg\bigwedge\Gamma\sigma_{\delta}$, taking $\Gamma \to \ $ as $C$.
\end{proof}



